Vyasa: A High-Performance Vectorizing Compiler for Tensor Convolutions on the Xilinx AI Engine

Xilinx's AI Engine is a recent industry example of energy-efficient vector processing that includes novel support for 2D SIMD datapaths and shuffle interconnection network. The current approach to programming the AI Engine relies on a C/C++ API for vector intrinsics. While an advance over assembly-level programming, it requires the programmer to specify a number of low-level operations based on detailed knowledge of the hardware. To address these challenges, we introduce Vyasa, a new programming system that extends the Halide DSL compiler to automatically generate code for the AI Engine. We evaluated Vyasa on 36 CONV2D and 6 CONV3D workloads, and achieved geometric means of 7.6 and 23.3 MACs/cycle for 32-bit and 16-bit operands (which represent 95.9% and 72.8% of the peak performance respectively). For 4 of these workloads for which expert-written codes were available to us, Vyasa demonstrated a geometric mean performance improvement of 1.10x with 50x smaller code relative to the expert-written codes.

==> tex/Challenges.tex <==
\section{Challenges} \label{sec:challenges}

Generating optimized libraries for convolutions on an AI Engine involve two key steps -- 1) Generating efficient code for a given schedule, and 2) Finding an optimal schedule that achieve close to the peak performance.    
We consider the convolution of a 4x3 filter on a 2D image expressed using Halide language~\cite{ragan2013halide}(shown in~\cref{fig:motivating-example}) as a motivating and running example to illustrate major challenges involved in generating optimized libraries.

\begin{figure}[!htb]
\centering
\begin{lstlisting}[language=C,escapeinside={@}{@}]
Buffer<int16> I(W, H);
Buffer<int16> W(4,3);
Var x, y;
RDom r(4, 3);
Func O; //output

//Description of the convolution computation
O(x,y) += W(r.x, r.y) * I(x+r.x, y+r.y);
\end{lstlisting}
\caption{Algorithmic description of the convolution of a 4x3 filter over an input 2D image in Halide language~\cite{ragan2013halide}.}
    \label{fig:motivating-example}
\end{figure}

\subsection{Generating Efficient Code for a Given Schedule} \label{subsec:challenges-generate-efficient-code}

As described in the background, the AI Engine architecture is heavily optimized for energy efficiency and silicon density, and as a result, the architecture doesn't have support for features found in traditional vector hardwares such as unaligned vector loads/stores, data manipulation units, scalar broadcast, and also 1D array of multipliers.
So, these constraints pose a new set of challenges to compilers/programmers in using the architecture for high-performance, and we illustrate these challenges with an example schedule (shown in~\cref{fig:motivating-example-after-lowering}) on the convolution example (shown in~\cref{fig:motivating-example}).  
The schedule involves unrolling loops corresponding to the filter width and height, and also vectorizing the loop corresponding to the output image width. 

\begin{figure}[!htb]
    \centering
    \begin{lstlisting}[language=C,escapeinside={@}{@}]
//A sample schedule
//Unrolling loops corresponding to filter dimensions
//Vectorizing loop corresponding to image width
O.update().unroll(r.x, 4).unroll(r.y,3)
     .vectorize(x, 16);

//Intermediate code after lowering
for y:
 for x: (vectorized)
   O(x:x+15,y) += W(0:0,0) * I(x:x+15,y);
   O(x:x+15,y) += W(1:1,0) * I(x+1:x+16,y);
   O(x:x+15,y) += W(2:2,0) * I(x+2:x+17,y);
   ......
   O(x:x+15,y) += W(3:3,2) * I(x+3:x+18,y+2);
    \end{lstlisting}
    \caption{A sample schedule for the convolution in~\cref{fig:motivating-example}, and the corresponding intermediate code (simplified) after lowering.}
    \label{fig:motivating-example-after-lowering}
\end{figure}

{\bf 1) Unaligned loads/stores:} The vector loads and stores in the AI Engine must be aligned to 128-bit memory boundaries.
For instance, assume that the {\tt I} array is aligned to 128-bit memory boundary, then the vector loads corresponding to {\tt I}, such as {\tt I(x+1:x+9, y), I(x+2:x+10, y)} are unaligned as they away by 32 and 64 bits from the 128-bit boundary.
Currently, the AI Engine architecture doesn't have vector instructions to perform unaligned loads, unlike modern AVX vector instructions in x86 hardware.

Alternatively, unaligned loads are typically addressed by loading two consecutive vector slots from memory, and combine them using data manipulation instructions such as shuffle, which again AI Engine don't have for energy efficiency and silicon density reasons. 
In addition, most of the prior compiler techniques~\cite{ragan2013halide} based on the previous approaches, i.e., unaligned vector instruction, consecutive loads and manipulation, overlooked partial vector reuse present among adjacent vector loads (e.g., {\tt I(x:x+8, y)} and {\tt I(x+1:x+9, y)}).


In addition to having unaligned vector loads in the convolutions, there do exists scalar loads such as {\tt filter(0,0)} which needs to be broadcasted into a vector register for performing vector MAC operation.
But, AI Engine architecture doesn't have support for performing broadcast operation, unlike traditional vector hardware units. 
The absence of support for unaligned load/store, broadcast operations poses difficulties to existing auto-vectorization techniques, and new analyses and transformations are required to address them within the constraints of architectural features.


{\bf 2) Modern SIMD Unit:} The SIMD unit present in the AI Engine, i.e., a 2D array of multipliers, is different from the regular SIMD units (1D array) in traditional vector hardware, as each lane (row) of the 2D array can perform more than one operation and also can reduce results from the operations along all columns of the lane.  
For the regular SIMD units, a MAC operation in a statement is translated directly into a vector MAC instruction, where as, for the AI Engine, there isn't a vector MAC instruction that only works for a row of the 2D array. 
As a result, new analysis and transformations such as fusing multiple vector MAC operations, that contribute to same output via "accumulation/reduction" property, to fit into 2D array are required to leverage data-parallelism. 



{\bf 3) Ineffective auto-interleaving:} The AI Engine compiler tools perform pre-processing transformations such as statement reordering to enable better software pipelining of loops to leverage instruction-level parallelism.
But, the existing compiler tools have challenges in reordering memory loads/stores/MAC operations because of the conservative treatment of memory operations during the dependence analysis.
As a result, additional analysis and transformations are required at the high-level to  interleave stores/loads/MAC operations in the loop body so that the downstream compilers can do pipelining effectively.


\subsection{Finding Optimal Schedules}
\label{subsec:challanges-finding-optimal-schedules}

The memory footprint of DNN convolution layers typically don't fit into the 32KB data memory of an AI Engine, and tiling strategies are required to fit into the data memory. 
In addition, the convolution layers often have a wide range of layer sizes, for, e.g., early layers have larger resolution compared to late layers and point-wise convolution have 1x1 filter sizes, and not one single tiling strategy is good for all possible convolutional layer sizes. 
As a result, our approach builds a library of highly efficient implementations of various convolution operators with various tile sizes that fit into the AI Engine data memory, and allow the high-level compiler to use the implementations in the library as primitives for running entire convolution operator and also the entire model.
Our approach generates optimized libraries for a convolution operation on an AI Engine by 1) finding an optimal schedule for each tile size of the convolution operation that fit into an AI Engine data memory, 2) generating efficient code for each optimal schedule, and finally 3) picking codes that reach close to peak performance to be used by a high-level compiler that can stitch them for multiple AI Engines. 
However, there exist following challenges in generating optimized libraries. 

{\bf Large search space:} The search space of schedules of a convolution operation on a given tile sizes include various loop transformations on the loop nest and data-layout transformations of convolution tensors.
Loop transformations include loop reordering, loop unroll and jam, loop selection for vectorization, and data-layouts transformations include data dimension reordering and data tiling.
On an average, the size of the search space of schedules of a 2D convolution operation (7D loop nest) for a given tile size is $10^{15}$, and searching for an optimal schedule is really challenging.





\iffalse 

\newpage

\begin{figure*} [!htb]
\centering
\includegraphics[width=\linewidth]{images/pldi-xhalide.pdf}
\end{figure*}

%\section{Motivating Example}\label{sec:motivating-example}
\section{Challenges}\label{sec:challenges-in-code-generation}

To motivate our approach, we consider the convolution of a 3x3 filter on a 2D image, whose algorithmic description in Halide language is shown in~\cref{fig:3x3filter-2Dimage}, and this convolution is commonly used in image processing pipelines and convolutional neural networks.
%
Using the motivating example, we illustrate the challenges in optimizing convolutions specific to the AIE core.
%
%In addition, we also briefly discuss performance issues in the c-codes generated by the Halide framework C code generator.

\begin{figure}[!htb]
\centering
\begin{lstlisting}[language=C,escapeinside={@}{@}]
Buffer<int16> I(W, H);
Buffer<int16> filter(3,3);
Var x, y;
RDom r(3, 3);
Func output;

//Description of the convolution computation
output(x,y) += filter(r.x, r.y) * I(x+r.x, y+r.y);
\end{lstlisting}
\caption{Algorithmic description of the convolution of a 3x3 filter over an input 2D image in Halide language~\cite{ragan2013halide}.}
    \label{fig:3x3filter-2Dimage}
\end{figure}


\begin{figure}[!htb]
    \centering
    \begin{lstlisting}[language=C,escapeinside={@}{@}]
//Sample schedule description
output.update().unroll(r.x, 3).unroll(r.y,3)
     .vectorize(x, 8);
//Halide IR (simplified) based on the above schedule
for y:
 for x: (vectorized)
   output(x,y) += filter(0,0) * image(x,y);
   output(x,y) += filter(1,0) * image(x+1,y);
   output(x,y) += filter(2,0) * image(x+2,y);
   ......
   output(x,y) += filter(3,3) * image(x+3,y+3);
    \end{lstlisting}
    \caption{Schedule description of the convolution in~\cref{fig:3x3filter-2Dimage}, and the corresponding  Halide IR (simplified) after lowering.}
    \label{fig:3x3filter-2Dimage-Halide-IR}
\end{figure}

%

Consider a sample schedule (shown in~\cref{fig:3x3filter-2Dimage-Halide-IR}) of the convolution, i.e., unrolling loops corresponding to filter width ({\tt r.x}), filter height ({\tt r.y}), and vectorizing the loop {\tt x} with a vector length of 8.
%
After lowering the high-level specification of convolution along with the schedule into Halide IR, the following are some of the main challenges in generating code specific to the AIE core from the Halide IR, and these challenges remain for other schedules as well.


{\it 1) Lack of hardware support for unaligned vector loads \& scalar broadcasts:} The vector loads and stores in the AIE core are aligned to 128-bit memory boundaries.
%
Even if starting address of the input image is aligned to 128-bit memory boundary, there exist vector loads in the Halide IR which are unaligned, for e.g., {\tt image(x+1, y)}.
%
Conventional x86 SIMD units have hardware support for unaligned loads either via special instructions (e.g., TODO) or  register-to-register data shuffling units (e.g., TODO), and the auto-vectorizing compilers (such as ICC) map the unaligned loads present in the computation as per the hardware support.
%
But, the AIE core doesn't have special instructions for unaligned loads, and also no data shuffling units for energy efficiency reasons, and as a result, the existing compiler techniques (TODO) are not directly applicable anymore.
%
However, the AIE core has a permute unit which is a shuffle network to arbitrarily select elements from a vector register whose size can be greater than vector length.
%
Our approach generates a larger aligned vector load that contains the required elements, and then using shuffle network of the permute unit to index into larger vector register to realize unaligned loads.


The Halide IR corresponding to the schedule ( in~\cref{fig:3x3filter-2Dimage-Halide-IR}) involves scalar loads (for, e.g., {\tt filter(0,0)}), and the Halide compiler and other compilers (such as ICC) typically broadcast the scalar value into a vector register to perform a vector operation.
%
But, the AIE core doesn't have an instruction to perform scalar broadcast into a vector register, again for energy efficiency reasons.
%
We address the above challenge using the permute unit by performing a vector load involving the scalar value, then indexing that scalar value in the vector register using the shuffle network for all vector lanes.


\noindent
{\it 2) 2D Vector multiplier array:} Since traditional x86 SIMD units handle only one vector arithmetic operation at a time, past compiler technologies map each vector arithmetic operation to its corresponding vector instruction.
%
However, AIE core has a 2D vector hardware, which is capable of performing more than one vector MAC operation and also do reduction along each lane.
%
As a result, mapping naively the code snippet to the 2D vector hardware results in under utilization of the hardware.


{\it Inefficient software pipelining:}

\fi

==> tex/Schedules.tex <==
\section{Our Approach for Finding Optimal Schedules} 
\label{sec:finding-optimal-schedules}
\newpage

